Fast Interactive Object Annotation with Curve-GCN

Manually labeling objects by tracing their boundaries is a laborious process. In Polygon-RNN++ the authors proposed Polygon-RNN that produces polygonal annotations in a recurrent manner using a CNN-RNN architecture, allowing interactive correction via humans-in-the-loop. We propose a new framework that alleviates the sequential nature of Polygon-RNN, by predicting all vertices simultaneously using a Graph Convolutional Network (GCN). Our model is trained end-to-end. It supports object annotation by either polygons or splines, facilitating labeling efficiency for both line-based and curved objects. We show that Curve-GCN outperforms all existing approaches in automatic mode, including the powerful PSP-DeepLab and is significantly more efficient in interactive mode than Polygon-RNN++. Our model runs at 29.3ms in automatic, and 2.6ms in interactive mode, making it 10x and 100x faster than Polygon-RNN++.

==> dataset.tex <==
%!TEX root = top.tex
\section{The MovieGraphs Dataset}
\label{sec:dataset}

% We begin discussing our MovieGraphs dataset by describing the annotation tool and data collection process, analyze the dataset, then discuss the results of our analysis.

% \paragraph{Workflow:} The annotators add character nodes by selecting the character's name from a list drawn from the IMDb character list. They can also add characters that are not on the list, by choosing \textit{unlisted character} and then naming it. The annotators then add other nodes as they watch the clip and see, hear or infer the topics, reasons, emotional and mental states of the characters. To ensure insight into the reasons behind each character's actions, one annotator works on each movie from start to finish.  Annotators also ground the graph into the video and dialog data by adding time stamps to interactions and many attributes.

% \paragraph{Situation Labeling Interface.} Our custom annotation tool provides three separate windows, where, for each clip, the worker provides:

% \begin{itemize}
% \item Scene label – provides information about the location where the situation takes place, e.g. a bar, living room, airport.
% \item Situation label – corresponds to the high-level topic of the clip. This is a summary of the type of social interactions that occur between the characters, e.g. wedding, first day at school.
% \item Description – explains in natural language what happens in the clip.
% \end{itemize}

% Good data for this part requires proper identification of the scene and situation, and a description that is thorough enough that people reading it can understand what happens in the clip.

% \paragraph{Training annotators on Upwork.} We hired annotators through the crowdsourcing service Upwork. Therefore, our setup had to overcome some unique challenges, the main one being uniformity: the annotators have to agree on the level of detail they put in the graph. To support data quality, we trained annotators on exactly the same clips, and continued monitoring the annotations. 

% \paragraph{Dividing Movies into Clips.}  To obtain the clips for annotation, we automatically split each movie into scenes ~\cite{Tapaswi2014_StoryGraphs} and then grouped the scenes into clips manually, while watching the movie, such that each clip corresponds to one social situation. As some situations were longer than others, our clips vary in length from around 20 seconds to 2 minutes. 

We construct a dataset to facilitate machine understanding of real-world social situations and human behaviors.   %, and of stories.
%We use movies as a proxy for the real world because they revolve around humans, and follow a natural timeline.
We developed a web-based annotation tool that allows human annotators to create graphs of arbitrary size by explicitly creating nodes and connecting them via a drag-and-drop interface. One annotator creates an entire graph, not just a subset of nodes. The benefit of our approach is that it ensures that each graph is \textit{globally coherent} (i.e., the emotions, interactions, topics, etc. make sense when viewed together). In addition, one of the key points of our dataset is that each annotator annotates a complete movie. This ensures that the graphs for \textit{consecutive clips} in a movie are \textit{coherent}---this would not be possible if annotators simply annotated randomly-assigned clips from a movie. We annotated \nmovies movies.
%To the best of our knowledge, this dataset is the first to contain graphs directly created by humans---this is in contrast to the Visual Genome dataset~\cite{krishna2016visual}, where graphs are created by fusing independent pairwise relationships.
%We annotated \nmovies movies, with the help of only a few annotators hired through the crowdsourcing service Upwork.
% % Each movie underwent a series of pre-processing steps.
Each movie was first split into scenes automatically~\cite{Tapaswi2014_StoryGraphs} and boundaries were refined manually, such that each clip corresponds to one \textit{social situation}.
We define a situation below.
% % In particular, we initially computed automatic scene boundaries via~\cite{Tapaswi2014_StoryGraphs}.
% %We define situations based on the intuitive human understanding of what constitutes a situation (\eg~robbery, first date).
% % Then, two annotators watched each movie and decided which shots to include in each clip.
% % The average durations of the clips are shown in Table~\ref{table:statstable}.
% %The average durations of the clips are shown in Table~\ref{table:statstable}.

% % We describe our annotation interface through the kind of information we were collecting.
% Next we describe in detail the components of our annotations.
% We then provide details on data collection, and finally present the statistics of the MovieGraphs dataset.


% %Our dataset consists of \nclips clips from \nmovies movies. Each clip shows one semantically coherent \emph{situation}. % based on the intuitive human understanding of what constitutes a situation.
% %We define a situation as a short event involving the same group of characters, where the nature of their interaction can be described with a single high-level topic, \eg, a \emph{robbery}, \emph{first date}, \emph{work-related disagreement}. %In movies, the situations are on average \SF{XX min} long.

% %We annotate each clip with: 1) a scene label; 2) situation label, 3) a situation graph; 4) a natural language description, 5) we label face tracks with identities of characters. Fig.~\ref{fig:openingexample} shows an example of an annotation for a video clip. The {\bf scene label} indicates the location where the situation takes place, \eg a \emph{bar}, \emph{living room}, \emph{airport}. The {\bf situation label} corresponds to the high-level topic of the clip. The {\bf description} provides a summary of what happened in the clip. We next describe the situation graphs, and the annotation workflow. We describe 5) in Subsec.~\ref{sec:collection}.

\begin{figure*}[t]
\centering
    % \includegraphics[height=0.495\linewidth,width=4cm,angle=90,origin=c]{../doc/images/Top20Emotions.pdf}
    % \includegraphics[height=0.495\linewidth,width=4cm,angle=90,origin=c]{../doc/images/Top20Interactions.pdf}\\[-14mm]
    % \includegraphics[height=0.495\linewidth,width=4cm,angle=90,origin=c]{../doc/images/Top20Relationships.pdf}
    % \includegraphics[height=0.495\linewidth,width=4cm,angle=90,origin=c]{../doc/images/Top25Scenes.pdf}\\[-17mm]
    %\includegraphics[width=0.3\linewidth]{../doc/images/Top20Emotions.pdf}
    %\includegraphics[width=0.3\linewidth]{../doc/images/Top20Interactions.pdf}
    %\includegraphics[width=0.3\linewidth]{../doc/images/Top20Relationships.pdf}

    % \includegraphics[height=6cm]{../doc/images/EmotionDistributionWithPics.pdf}\hspace{2mm}
    % \includegraphics[height=6cm]{../doc/images/InteractionDistributionWithPics.pdf}\hspace{2mm}
    % \includegraphics[height=6cm]{../doc/images/SituationDistributionWithPics.pdf}

    % TODO: Add pictures to these distribution images.
    \includegraphics[height=6cm]{stats/current_stats/Top25EmoAttributes.pdf}\hspace{2mm}
    \includegraphics[height=6cm]{stats/current_stats/Top25IntersAndSummaries.pdf}\hspace{2mm}
    \includegraphics[height=6cm]{stats/current_stats/Top25Situations.pdf}
\caption{\small Distributions of the top 15 emotional attributes,  interactions, and situations.}
\label{fig:distributions}
\end{figure*}

\subsection{Annotation Interface}
Our annotation interface allowed the annotator to view clips sequentially. For each movie clip, the annotator was asked to provide information about the scene and situation, write a natural language description and create a detailed graph of the situation Fig.~\ref{fig:openingexample}. We describe each component of the annotation:

\textbf{Scene label} provides information about the location where the situation takes place, \eg \textit{bar, living room, airport}.

\textbf{Situation label} corresponds to the high-level topic of the clip and is a summary of the type of social interactions that occur between characters, \eg \textit{robbery, party}.
%as a short event involving a fixed group of characters, where the nature of their interaction can be described with a single high-level topic, \eg, a \emph{robbery}, \emph{first date}, or \emph{party}.

\textbf{Description} provides a natural language explanation of what happens in the clip. It consists of several sentences written in English.

\textbf{Graphs} represent a human's understanding of a given situation. Our graphs feature 8 different types of nodes that the annotators can add to a canvas, and draw \textit{edges} between them to indicate dependencies. Note that we allow the annotator to choose the \textit{directionality} of the dependency by orienting the edges between nodes. A graph consists of the following \textit{nodes}:

\textbf{Character} nodes represent the people in each scene. %These typically contain the names of characters obtained from the IMDb movie database~\footnote{\url{http://www.imdb.com/}}.
The interface provides a comprehensive list of character names obtained from IMDb\footnote{\url{http://www.imdb.com/}}, which the annotators can drag and drop onto the graph's canvas.
We also allow new characters to be added.

\textbf{Attributes} are added to character nodes. These attributes can be constant, such as age, gender, ethnicity, orientation, appearance, or can vary, such as mental and emotional states.
    % # attribute sub-types: 'tim', 'age', 'gen', 'ori', 'eth', 'app', 'pro', 'emo'

\textbf{Relationship} nodes can link two or more characters.
The relationships can refer to: family (\eg~\emph{parent}, \emph{spouse}), friendship/romance (\eg~\emph{friend}, \emph{lover}), or work (\eg~\emph{boss}, \emph{co-worker}).
%Some relationships are constant throughout a movie, \eg parent-child.
%Relationships that start and end at different points in the movie (\eg,~people become friends or enemies) are tagged with an start/end token indicating whether the relationship is starting or terminating in the given scene.
A relationship node can be tagged with a start/end token indicating whether the relationship starts or ends in a given clip (\eg the \emph{spouse} relationship starts in a \textit{wedding} clip). Otherwise, we assume that the characters are already in the relationship prior to the scene (\eg they were already married). %For example, \emph{spouse} can start if the scene shows a wedding.

\textbf{Interaction} nodes can be added to link two or more characters. %to describe the types of interactions that occur between them. %The interactions between characters are defined
Interactions are either verbal (\eg \emph{suggests}, \emph{warns}) or non-verbal ways of communication (\eg \emph{hugs}, \emph{sits near}).  They can be directed (pointing from one character to another, \eg \emph{A helps B}), or bidirectional if the  interaction is symmetric (\eg \emph{A and B argue)}.
%Note that we make a distinction between two types of interaction nodes. A \emph{local interaction} indicates an interaction that is typically shorter in duration, while the \emph{summary interaction} describes a high-level semantic label of the interaction. For example, a scene with a mother asking her son about an upcoming trip may contain several \emph{asks about-topic} local interactions, while the summary interaction from mum to son is \emph{worries about}. Typically there is a single directed summary interaction pointing from each character to the other, while there may be many local ones.

\textbf{Topic} nodes can be added to interactions to add further detail. For example, \textit{suggests} (interaction) can be linked to \textit{to quit the job} (topic).

% Each interaction can optionally be linked with a topic node which provides further detail about the interaction. For example, \emph{suggests} could be linked to a topic \emph{to quit the job}.


\textbf{Reason}
%Both attribute and interaction nodes can also be optionally linked with reason nodes which provide an \emph{explanation} for why the character may be experiencing a certain emotion or why she/he is engaging in a particular interaction.
nodes can be added to interactions and attributes to provide an explanation. For example, \textit{apologizes} (interaction) can be linked to \textit{he was late} (reason). Reasons can also be added to emotions. For example, \textit{happy} (emotion) can be linked to \textit{she got engaged} (reason).
Reason nodes contain \textit{inferred} common-sense information.

\textbf{Action} nodes can be added to characters to describe what the character does without involving another character (\eg \textit{slams the door, drinks whiskey}).

\textbf{Time stamp} nodes ground the graph in the video clip, providing the interval when an interaction occurs (\eg a character \textit{dances} with another) or how long an emotional state lasts (\eg a character is \textit{sad} for a while, then (s)he becomes \textit{happy}) within the same clip.

%Fig.~\ref{fig:openingexample} shows an example of an annotation for a video clip. Dataset statistics is shown in Table~\ref{table:statstable}.
%The situation graph represents a human's understanding of a movie clip.
%It contains characters present in the scene and the interactions inferred between them, as well as their emotions.



% \begin{table}[t]
% % \vspace{-4mm}
% \centering
% \small
% \tabcolsep1.2mm

% \label{table:statstable}
% \begin{tabular}{lcccc}
% \toprule
%                  & TRAIN & VAL  & TEST    & TOTAL    \\
% \midrule
%  Movies          & 22    & 4    & 7       & 33       \\
%  Clips           & 3093  & 630  & 890     & 4613     \\
%  Duration (s)    & 46.3  & 39.5 & 48.5    & 45.8     \\
%  Desc. \#Words   & 32.8  & 33.4 & 30.2    & 32.4     \\
%  Desc. \#Sents   &  2.8  &  2.5 &  2.5    &  2.7     \\
%  Characters      &  3.0  &  2.9 &  3.0    &  3.0     \\
%  Interactions    &  3.6  &  2.4 &  3.6    &  3.4     \\
%  Relationships   &  3.5  &  2.6 &  3.5    &  3.4     \\
%  Attritutes      & 13.4  & 13.3 & 14.1    & 13.6     \\
%  Topics          &  2.2  &  2.4 &  2.3    &  2.2     \\
%  Reasons         &  1.1  &  1.6 &  1.0    &  1.1     \\
%  Timestamps      &  2.7  &  3.2 &  2.9    &  2.8     \\
% \bottomrule
% \end{tabular}


\begin{table}[t]
% \vspace{-4mm}
\centering
\small
\tabcolsep1.2mm

\label{table:statstable}
\input{stats/current_stats/stats_table.tex}

\vspace{2mm}
\caption{\small
Statistics of the MovieGraphs dataset across train, validation, and test splits.
We show the number of movies and clips; their average duration; the number of words and sentences in description;
and average counts for different types of nodes in each scene: characters, interactions, relationships, attributes, topics, reasons.}

\end{table}


% \vspace{-3mm}
\subsection{Data Collection Procedure}
\label{sec:collection}
% \vspace{-1mm}
We hired workers from the crowdsourcing website Upwork. We worked closely with a small set of annotators, to ensure high-quality annotations. Each worker went through a training phase in which they annotated the same set of clips according to an instruction manual. We provided them with detailed feedback, to calibrate their annotations (i.e., ensure that they had similar levels of detail, and that all of the aspects of the situations were captured by the graphs they created).
%: first, we asked them to read through a document containing annotation instructions (16 pages?); then, we asked them to annotate three clips from the movie ``27 Dresses''; after they annotated the clips, we provided them with detailed feedback, to calibrate their annotations (i.e., ensure that they had similar levels of detail, and that all of the aspects of the situations were captured by the graphs they created).
%Each crowdworker annotated a full movie at a time to ensure that the annotations are consistent across multiple scenes in the movie. For each clip, an annotator: 1) watched the clip; 2) wrote scene and situation labels; 3) wrote a natural-language description; and 4) created a graph to capture the details of the situation.

% We communicated with the annotators throughout the data collection process; we checked on the annotations for each movie periodically, and provided feedback when necessary. Annotators could also ask us questions if a particularly complex situation arose. This was done to ensure quality.

We also had a \textit{cross-checking} phase, where annotators swapped movies and checked each others' work.
%In this phase, annotators were asked to check that each of the interaction, emotions, topics, and reasons made sense, that nothing important was missing, and that spelling was correct.
%; they were instructed to correct any of these issues.
% %\subsection{Data Collection Method}
% %\label{subsec:data_collection}

% %The clips are then annotated by UpWork annotators, who watch each clip and assign it scene and situation labels.
% %Then, the annotator describes what happens in that clip, in natural language.
% %Finally, the annotator creates a graph describing the clip.
% %An annotator can include in the graph nodes corresponding to: characters, relationships and interactions between characters, attributes of characters, and reasons for the interactions.
% %We provide initial vocabularies for each node type which users can select from, but they can also add custom items to the lists.

% % Each annotator annotated every scene, by following the movie from start to end.
% % We asked the annotators to not peek at what happens next in the movie but rather annotate what they are seeing as they are watching the movie.
% Each annotator watched a movie from start to finish, annotating each clip in order.
% This ensured that each annotation contained data inferred from the movie up until that point in time.
% The typical workflow of the annotator was to watch the scene and first write the description in natural language, then provide the scene and situation label, and finally create the graph.
% %To annotate the situation graphs, annotators first selected characters from lists obtained from IMDb, and then added the other nodes by linking them to the corresponding characters.
% We provide initial vocabularies for scenes and situations which users could select from, but they were also allowed to add custom items to the lists. %\SF{Can we comment on sizes of vocabularies, initial vs final?}
% The interactions, topics, and reasons were free-form, but we encouraged the annotators to be concise. %We also enabled  time-stamping  the attribute and interaction nodes. This was time consuming to do, and only a subset of nodes have this information.

% %To capture diversity in natural language summaries of clips, as well as to ensure that the information in the graph and the summary are not correlated (written by same annotator), we had another, independent annotator write additional clip summaries for each movie. This annotator had no access to the information provided by the first annotator.

% Each annotator handled an average of 10 movies, and each movie annotation was cross-checked by another annotator.
% We went over half the movies, making sure that the natural language descriptions were error-free.
% %We also \textit{canonicalized} the node labels by manually creating mappings to correct misspellings, and to merge together semantically similar labels.

% \subsection{Data Collection for Face ID}
% \label{sec:collection}
% % \vspace{-1mm}
% We additionally grounded each character in the graph with all the face tracks in the clip (obtained with OpenFace~\cite{baltruvsaitis2016openface}).
% As there are on average 1750 face tracks per movie (12 per clip, and over 57K in our full dataset), annotating the tracks directly would have been time consuming.
% Instead, we first linked face tracks that belong to the same person in a clip by performing hierarchical agglomerative clustering on upper body color histogram features (a character wears the same clothing during a clip) corresponding to the face tracks.
% %To do this, we extract the VGG-16~\cite{parkhi2015deep} features in each track and perform hierarchical agglomerative clustering  on the track-track distances.
% The annotator is then asked to assign character names (from those found in the graph) to clusters in the clip. In cases when clustering is wrong, we break the cluster into face tracks, and the annotator labels each track. We did this for 3384 out of 17688 clusters.
% %Further details are in Suppl. mat.

% \vspace{-3mm}
\subsection{Dataset Statistics}
\label{subsec:statistics}
% \vspace{-1mm}


% \begin{figure}[t]
% % \vspace{-2mm}
% \centering
% \begin{tabular}{cc}
%    (a)  \includegraphics[height=3.cm,trim=0 90 0 90,clip]{../doc/images/AttributeTypesPie.pdf}  & (b) \includegraphics[height=3.cm,trim=0 0 0 00,clip]{../doc/images/radar_plots/tt1285016.pdf} \\
%     \end{tabular}
%     % \vspace{-2mm}
% \caption{\small (a) Proportions of attributes types. (b) Character emotional profiles from ``The Social Network.''}
% \label{fig:socialnetwork_emotions}
% % \vspace{-3mm}
% \end{figure}


\begin{figure}[t]
% \vspace{-2mm}
\centering
   % \includegraphics[width=\linewidth]{../doc/images/radar_plots/tt1285016.pdf}
   \includegraphics[width=\linewidth]{images/radar_plots/tt1285016.pdf}
\caption{\small Character emotional profiles from ``The Social Network.''}
\label{fig:socialnetwork_emotions}
% \vspace{-3mm}
\end{figure}



%In this section we present a statistical analysis of the data collected for \nmovies movies.
Our dataset consists of \nclips annotated clips from \nmovies movies. A summary of the dataset statistics is shown in Table~\ref{table:statstable}.
%\vspace{-3mm}
%\paragraph{Analysis of individual nodes.} %Fig.~\ref{fig:scenecharacterdistribution}(a) shows the distribution of the number of characters that appear per scene, across all movies.
The majority of clips contain between 2 and 4 characters, and a graph has on average 13.6 attributes and 3.4 interactions. Fig.~\ref{fig:distributions} plots distributions of the top 15 emotion attributes, interactions, and situations. Fig.~\ref{fig:socialnetwork_emotions} shows the emotional profiles of the characters from the movie ``The Social Network''.
%Our dataset additionally has 57,752 face tracks labeled with character names.
%A graph has on average 3.3 relationships, with more details about the number of relationships per scene shown in Fig.~\ref{fig:relationshipdistribution} (a).



% \vspace{-3mm}
%\paragraph{Correlations between nodes.}
%\label{subsec:data_correlations}
%In the following analysis, the area of each circle is proportional to the number of co-occurrences of the corresponding values in the x- and y-axes.
We show correlations between nodes for a selected set of labels in Fig.~\ref{fig:Correlations} and discuss them below:
%{\bf Interactions and Emotions:}
\textbf{Interactions and Emotions:}
The plot shows that certain emotions are correlated with certain interactions.
For example, when someone is \textit{angry}, he/she is most likely to \textit{yell, ask, inform}, or \textit{hit} another person.
Also, a person who \textit{hugs} is likely to be \textit{loving}, \textit{sad}, or \textit{scared}. 
%{\bf Relationships and Emotions:}`'
\textbf{Relationships and Emotions:}
The plot shows which emotions are most prevalent in various relationships.
For example, \textit{hostages} are often \textit{scared}, and \textit{parents} are mostly \textit{loving}, \textit{sad}, or \textit{angry}.
%{\bf Interactions and Interactions:} Fig.~\ref{fig:Correlations} shows what one character does in response to another person's actions.
%For example, when one person hugs, the other person usually hugs back, and/or apologizes, flirts, or gives advice.
%{\bf Situations and Interactions:}
\textbf{Situations and Interactions:}
As expected, people engage in different interactions depending on the situation.
The plot shows that, for example, people at a \textit{party} are likely to \textit{dance, kiss}, and \textit{watch other people}, while people in an \textit{intimate situation}, \textit{kiss}.
%{\bf Situations and Scenes.}
\textbf{Situations and Scenes:}
Different social situations occur in different places.
As shown in the plot, parties and weddings happen at different venues: a \textit{party} usually occurs in a \textit{house} or a \textit{bar}, while a \textit{wedding} usually takes place in a \textit{church} or at a \textit{restaurant}.


\begin{figure*}[t]
% \vspace{-2mm}
\centering
\includegraphics[height=4cm]{../doc/images/heatmaps/InteractionEmotionHeatmap.pdf}
\includegraphics[height=4cm]{../doc/images/heatmaps/RelationshipEmotionHeatmap.pdf}
\includegraphics[height=4cm]{../doc/images/heatmaps/SituationInteractionHeatmaps.pdf}
\includegraphics[height=4cm]{../doc/images/heatmaps/SceneSituationHeatmap.pdf}
% \vspace{-3mm}
\caption{\small Correlations between different types of social aspects of scenes.}%Correlations between interactions and emotions, emotions and relationships, interactions and situations, %interactions occurring between pairs of characters,
%and scenes and situations.}
\label{fig:Correlations}
% \vspace{-2mm}
\end{figure*}

